SGCCNet: Single-Stage 3D Object Detector With Saliency-Guided Data Augmentation and Confidence Correction Mechanism

The single-stage point-based 3D object detectors have attracted widespread research interest due to their advantages of lightweight and fast inference speed. However, they still face challenges such as inadequate learning of low-quality objects (ILQ) and misalignment between localization accuracy and classification confidence (MLC). In this paper, we propose SGCCNet to alleviate these two issues. For ILQ, SGCCNet adopts a Saliency-Guided Data Augmentation (SGDA) strategy to enhance the robustness of the model on low-quality objects by reducing its reliance on salient features. Specifically, We construct a classification task and then approximate the saliency scores of points by moving points towards the point cloud centroid in a differentiable process. During the training process, SGCCNet will be forced to learn from low saliency features through dropping points. Meanwhile, to avoid internal covariate shift and contextual features forgetting caused by dropping points, we add a geometric normalization module and skip connection block in each stage. For MLC, we design a Confidence Correction Mechanism (CCM) specifically for point-based multi-class detectors. This mechanism corrects the confidence of the current proposal by utilizing the predictions of other key points within the local region in the post-processing stage. Extensive experiments on the KITTI dataset demonstrate the generality and effectiveness of our SGCCNet. On the KITTI \textit{test} set, SGCCNet achieves $80.82\%$ for the metric of $AP_{3D}$ on the \textit{Moderate} level, outperforming all other point-based detectors, surpassing IA-SSD and Fast Point R-CNN by $2.35\%$ and $3.42\%$, respectively. Additionally, SGCCNet demonstrates excellent portability for other point-based detectors

==> Content/gallery.tex <==
%算法

% \begin{algorithm}
% 	\caption{My algorithm}\label{euclid}
% 	\begin{algorithmic}[1]
% 		\Procedure{MyProcedure}{}
% 			abc
% 		\State $\textit{stringlen} \gets \text{length of }\textit{string}$
% 		\State $i \gets \textit{patlen}$
% 		\BState \emph{top}:
% 		\If {$i > \textit{stringlen}$} \Return false
% 		\EndIf
% 		\State $j \gets \textit{patlen}$
% 		\BState \emph{loop}:
% 		\If {$\textit{string}(i) = \textit{path}(j)$}
% 		\State $j \gets j-1$.
% 		\State $i \gets i-1$.
% 		\State \textbf{goto} \emph{loop}.
% 		\State \textbf{close};
% 		\EndIf
% 		\State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
% 		\State \textbf{goto} \emph{top}.
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[h]
% 	\caption{An example for format For \& While Loop in Algorithm}
% 	\begin{algorithmic}[1]
% 		\For{each $i\in [1,9]$}
% 		\State initialize a tree $T_{i}$ with only a leaf (the root);
% 		\State $T=T\cup T_{i};$
% 		\EndFor
% 		\ForAll {$c$ such that $c\in RecentMBatch(E_{n-1})$}
% 		\label{code:TrainBase:getc}
% 		\State $T=T\cup PosSample(c)$;
% 		\label{code:TrainBase:pos}
% 		\EndFor;
% 		\For{$i=1$; $i<n$; $i++$ }
% 		\State $//$ Your source here;
% 		\EndFor
% 		\For{$i=1$ to $n$}
% 		\State $//$ Your source here;
% 		\EndFor
% 		\State $//$ Reusing recent base classifiers.
% 		\label{code:recentStart}
% 		\While {$(|E_n| \leq L_1 )and( D \neq \phi)$}
% 		\State Selecting the most recent classifier $c_i$ from $D$;
% 		\State $D=D-c_i$;
% 		\State $E_n=E_n+c_i$;
% 		\EndWhile
% 		\label{code:recentEnd}
% 	\end{algorithmic}
% \end{algorithm}

%示意图

% \begin{figure}
	% 	\centering  
	% 	\scriptsize  
	% 	\tikzstyle{format}=[rectangle,draw,thin,fill=white]  
	% 	%定义语句块的颜色,形状和边
	% 	\tikzstyle{test}=[diamond,aspect=2,draw,thin]  
	% 	%定义条件块的形状,颜色
	% 	\tikzstyle{point}=[coordinate,on grid,]  
	% 	%像素点,用于连接转移线
	% 	\begin{tikzpicture}%[node distance=10mm,auto,>=latex',thin,start chain=going below,every join/.style={norm},] 
	% 	%start chain=going below指明了流程图的默认方向，node distance=8mm则指明了默认的node距离。这些可以在定义node的时候更改，比如说 
	% 	%\node[point,right of=n3,node distance=10mm] (p0){};  
	% 	%这里声明了node p0，它在node n3 的右边，距离是10mm。
	% 	%第一个node \node[样式] (标号){内容} 
	% 	\node[format] (start){Start};
	% 	%后面的node,使用below of=标号,right of=标号,left of=标号,表示位置,可以加上node distance=xmm调节位置. 
	% 	\node[format,below of=start,node distance=7mm] (define){Some defines};
	% 	\node[format,below of=define,node distance=7mm] (PCFinit){PCF8563 Initialize};
	% 	\node[format,below of=PCFinit,node distance=7mm] (DS18init){DS18 Initialize};
	% 	\node[format,below of=DS18init,node distance=7mm] (LCDinit){LCD Initialize};
	% 	\node[format,below of=LCDinit,node distance=7mm] (processtime){Processtime};
	% 	\node[format,below of=processtime,node distance=7mm] (keyinit){Key Initialize};
	% 	\node[test,below of=keyinit,node distance=15mm](setkeycheck){Check Set Key};
	% 	\node[point,left of=setkeycheck,node distance=18mm](point3){};
	% 	\node[format,below of=setkeycheck,node distance=15mm](readtime){Read Time};
	% 	\node[point,right of=readtime,node distance=15mm](point4){};
	% 	\node[format,below of=readtime](processtime1){Processtime};
	% 	\node[format,below of=processtime1](gettemp){Get Temperature};
	% 	\node[format,below of=gettemp](display){Display All Data};
	% 	\node[format,right of=setkeycheck,node distance=40mm](setsetflag){Set SetFlag=1};
	% 	\node[format,below of=setsetflag](setinit){Set Mode Initialize};
	% 	\node[format,below of=setinit](checksetting){Checksetting()};
	% 	\node[test,below of=checksetting,node distance=15mm](savecheck){Check Save Key};
	% 	\node[format,below of=savecheck,node distance=15mm](clearsetflag){Clear SetFlag=0};
	% 	\node[format,below of=clearsetflag](settime){Set Time};
	% 	\node[point,below of=display,node distance=7mm](point1){};
	% 	\node[point,below of=settime,node distance=7mm](point2){};
	% 	%\node[format] (n0) at(4,4){A}; 直接指定位置 
	% 	%定义完node之后进行连线,
	% 	%\draw[->] (n0.south) -- (n1); 带箭头实线
	% 	%\draw[-] (n0.south) -- (n1); 不带箭头实线
	% 	%\draw[<->] (n0.south) -- (n1.north);   双箭头
	% 	%\draw[<-,dashed] (n1.south) -- (n2.north); 带箭头虚线 
	% 	%\draw[<-] (n0.south) to node{Yes} (n1.north);  带字,字在箭头方向右边
	% 	%\draw[->] (n1.north) to node{Yes} (n0.south);  带字,字在箭头方向左边
	% 	%\draw[->] (n1.north) to[out=60,in=300] node{Yes} (n0.south);  曲线
	% 	%\draw[->,draw=red](n2)--(n1);  带颜色的线
	% 	\draw[->] (start)--(define);
	% 	\draw[->] (define)--(PCFinit);
	% 	\draw[->](PCFinit)--(DS18init);
	% 	\draw[->](DS18init)--(LCDinit);
	% 	\draw[->](LCDinit)--(processtime);
	% 	\draw[->](processtime)--(keyinit);
	% 	\draw[->](keyinit)--(setkeycheck);
	% 	\draw[->](setkeycheck)--node[above]{Yes}(setsetflag);
	% 	\draw[->](setkeycheck) --node[left]{No} (readtime);
	% 	\draw[->](readtime)--(processtime1);
	% 	\draw[->](processtime1)--(gettemp);
	% 	\draw[->](gettemp)--(display);
	% 	\draw[-](display)--(point1);
	% 	\draw[-](point1)-|(point3);
	% 	\draw[->](point3)--(setkeycheck.west);
	% 	\draw[->](setsetflag)--(setinit);
	% 	\draw[->](setinit)--(checksetting);
	% 	\draw[->](checksetting)--(savecheck);
	% 	\draw[->](savecheck)--node[left]{Yes}(clearsetflag);
	% 	\draw[->](savecheck.west)|-node[left]{No}(checksetting);
	% 	\draw[->](clearsetflag)--(settime);
	% 	\draw[-](settime)--(point2);
	% 	\draw[-](point2)-|(point4);
	% 	\draw[->](point4)--(readtime.east);
	% 	\end{tikzpicture}  
	% \end{figure}

	% \begin{tikzpicture}
	% 	[every node/.style={align=center}]
	% 	\foreach \x in{1,2,3,4,5}
	% 	\fill[red!60](0,\x)circle(5pt)node(a\x){};
	% 	\fill[blue!60](-2,1.5)circle(5pt)node(b1){};
	% 	\fill[blue!60](-2,2.5)circle(5pt)node(b2){};
	% 	\fill[blue!60](-2,3.5)circle(5pt)node(b3){};
	% 	\fill[blue!60](-2,4.5)circle(5pt)node(b4){};
	% 	\fill[blue](2,3)circle(5pt)node(c){};
	% 	\node(y4)at(-3,4.5){$x_1$};
	% 	\node(y3)at(-3,3.5){$\vdots$};
	% 	\node(y2)at(-3,2.5){$x_n$};
	% 	\node(y1)at(-3,1.5){bias:1};
	% 	\node at(-2,6){Input\\layer};
	% 	\node at(0,6){Hidden\\layer};
	% 	\node at(2,6){Output\\layer};
	% 	\node(d)at(3.5,3){$N(x,p)$};
	% 	\draw[-stealth](c)--(d);
	% 	\foreach \x in{1,2,3,4}
	% 	\draw[-{stealth[sep=2pt]}](y\x)--(b\x);
	% 	\foreach \x in{1,2,3,4}
	% 	{\foreach \y in{1,2,3,4,5}
	% 		{\draw[-{stealth[sep=2pt]}](b\x)--(a\y);
	% 			\draw[-{stealth[sep=4pt]}](a\y)--(c.west);
	% 		}
	% 	}
	% 	\end{tikzpicture}
	
% 水印
% \AddToShipoutPicture{\BackgroundPicture} % 开始加入水印
% \ClearShipoutPicture % 停止使用水印

% 为避免矩阵求逆运算，$(\bm D-\bm L)^{-1}$也可以不求，写成
% $$
% \left\{\begin{array}{l}
% x_{1}^{(k+1)}=\dfrac{1}{4}\left(3+x_{2}^{(k)}\right) \\
% x_{2}^{(k+1)}=-1+x_{1}^{(k+1)}+x_{3}^{(k)} \\
% x_{3}^{(k+1)}=x_{2}^{(k+1)}
% \end{array}\right.
% ,\quad 
% \left(\begin{array}{ccc}
% 4 & 0 & 0 \\
% -1 & 1 & 0 \\
% 0 & -1 & 1
% \end{array}\right)\left(\begin{array}{c}
% x_{1}^{(k+1)} \\
% x_{2}^{(k+1)} \\
% x_{3}^{(k+1)}
% \end{array}\right)=\left(\begin{array}{c}
% 3 \\
% -1 \\
% 0
% \end{array}\right)+\left(\begin{array}{ccc}
% 0 & -1 & 0 \\
% 0 & 0 & -1 \\
% 0 & 0 & 0
% \end{array}\right)\left(\begin{array}{c}
% x_{1}^{(k)} \\
% x_{2}^{(k)} \\
% x_{3}^{(k)}
% \end{array}\right)
% $$

% \begin{table}[H]
%   \centering
% %   \caption{三线表示例}
%   \begin{tabular}{cccccc}
%     \toprule
%     $t_i$ & 1 & 2 & 3 & 4 & 5\\
%     \midrule
%     $z_i$ & 2 & 4 & 6.4 & 8 & 8.6\\
%     \bottomrule
%   \end{tabular}
% %   \label{tab:three-line}
% \end{table}

==> Content/titlepage.tex <==
\begin{titlepage}
%本页为自定义的封面
	% \title{作业标题}
	% \author{作者}
    
	\center
	\quad\\[1cm]
	\includegraphics[width=12cm]{Content/logo.jpg}\\[1.5cm]
% 	{\Large 题目1}\\[0.5cm]
% 	{\Large 题目2}\\[1.5cm] 
	\quad\\[1cm]
	\makeatletter
	{\linespread{4}\Huge\bfseries\@title}\\[2cm]
	\begin{table}[H]
		\centering
		  \begin{tabular}{rl}
			{\Large Name：}&{\Large Alan Liang}\\[0.5cm]
		  \end{tabular}\\
	\end{table}
	\makeatother
	\quad\\[1cm]
	{\Large \today}\\[2cm] % 日期
	\vfill 
\end{titlepage}

==> table/abb.tex <==
\begin{table}
\centering
\caption{Abbreviation explanation.}
\resizebox{3.5in}{!}{
\begin{tabular}{ll} 
\toprule
Full text                                                                                           & Abbreviation  \\ 
\hline
\textbf{Li}ght \textbf{D}etection \textbf{A}nd \textbf{R}anging                                     & LiDAR         \\
\textbf{I}nadequate learning of \textbf{L}ow-\textbf{Q}uality objects                               & ILQ           \\
\makecell[l]{\textbf{M}isalignment between \textbf{L}ocalization accuracy\\ and \textbf{C}lassification confidence} & MLC           \\
\textbf{I}nternal \textbf{C}ovariate \textbf{S}hif                                                  & ICS           \\
\textbf{S}ingle-\textbf{S}tage \textbf{D}etector                                                    & SSD           \\
\textbf{G}round \textbf{T}ruth                                                                      & GT            \\
\textbf{G}eometric \textbf{N}ormalization \textbf{M}odule                                           & GNM           \\
\textbf{S}aliency-\textbf{G}uided \textbf{D}ata \textbf{A}ugmentation                               & SGDA          \\
\textbf{C}onfidence \textbf{C}orrection \textbf{M}echanism                                          & CCM           \\
\textbf{B}ird's-\textbf{E}ye \textbf{V}iew                                                          & BEV           \\
\textbf{R}ange \textbf{V}iew                                                                        & FV            \\
\textbf{S}et \textbf{A}bstraction                                                                   & SA            \\
\textbf{I}ntersection\textbf{ o}ver \textbf{U}nion                                                  & IoU           \\
\textbf{A}verage \textbf{P}recision                                                                 & AP            \\
\textbf{M}ean \textbf{A}verage \textbf{P}recision                                                   & mAP           \\
\textbf{V}oxel \textbf{F}eature\textbf{ E}ncoding                                                   & VFE           \\
\textbf{F}arthest \textbf{P}oint \textbf{S}ampling                                                  & FPS           \\
\textbf{F}eature \textbf{F}arthest \textbf{P}oint \textbf{S}ampling                                 & F-FPS         \\
\textbf{D}ynamic \textbf{B}all \textbf{Q}uery                                                       & DBQ           \\
\textbf{M}ulti-\textbf{L}ayer\textbf{ P}erceptron                                                   & MLP           \\
\textbf{G}raph \textbf{N}eural \textbf{N}etwork                                                     & GNN           \\
\textbf{F}ully \textbf{C}onnected                                                                   & FC            \\
\textbf{W}eighted \textbf{C}ross\textbf{ E}ntropy                                                   & WCE           \\
\bottomrule
\end{tabular}}
\label{tab:10}
\end{table}


==> table/clc_dataset.tex <==
% \usepackage{color}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
	\centering
	\begin{tabular}{llll} 
		\toprule
		Split                       & \textcolor[rgb]{0.2,0.2,0.2}{Category} & Number  & \textcolor[rgb]{0.2,0.2,0.2}{Total~}  \\ 
		\hline
		\multirow{3}{*}{Train}      & Car                                    & $13382$ & \multirow{3}{*}{$16239$}              \\
		& Pedestrian                             & $2159$  &                                       \\
		& Cyclist                                & $698$   &                                       \\ 
		\hline
		\multirow{3}{*}{Validation} & Car                                    & $13874$ & \multirow{3}{*}{$17014$}              \\
		& Pedestrian                             & $2260$  &                                       \\
		& Cyclist                                & $880$   &                                       \\
		\bottomrule
	\end{tabular}
	\label{tab:5}
\end{table}

